Private Synthetic Data for Multitask Learning and Marginal Queries

We provide a differentially private algorithm for producing synthetic data simultaneously useful for multiple tasks: marginal queries and multitask machine learning (ML). A key innovation in our algorithm is the ability to directly handle numerical features, in contrast to a number of related prior approaches which require numerical features to be first converted into {high cardinality} categorical features via {a binning strategy}. Higher binning granularity is required for better accuracy, but this negatively impacts scalability. Eliminating the need for binning allows us to produce synthetic data preserving large numbers of statistical queries such as marginals on numerical features, and class conditional linear threshold queries. Preserving the latter means that the fraction of points of each class label above a particular half-space is roughly the same in both the real and synthetic data. This is the property that is needed to train a linear classifier in a multitask setting. Our algorithm also allows us to produce high quality synthetic data for mixed marginal queries, that combine both categorical and numerical features. Our method consistently runs 2-5x faster than the best comparable techniques, and provides significant accuracy improvements in both marginal queries and linear prediction tasks for mixed-type datasets.

==> docs/algos/framework.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% RAP
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{General Framework for Query Release}\label{alg:framework}
\begin{algorithmic}[1]
\Require A dataset $D$ with $n$ records.


\State \textbf{Input:} A class of statistical queries $Q$ ($Q$ might be infinite), $\rho$-zCDP Select Algorithm $\cM_{\rho}$.

\State \textbf{Parameters:} Learning rate parameter $\alpha>0$, private select epochs $T$, number of queries per epoch $m$, the size of the synthetic dataset $n'$, and zCDP parameter $\rho$.
%
\State Initialize $D'_0\in \cX^{n'}$, $Q_0 = \{\}$ and compute the privacy budget for each round.
\begin{align*}
    \rho' = \tfrac{1}{T m}
\end{align*}

    % \State Set $D'_{\text{best}}$ to $D'$ if $D'$ has lower error.
% \State $D'_{\text{best}} \in \argmin \{ D_{\sigma, \gamma} \}$.

\For{$t=1$ \textbf{ to } $T$}
    \State 1) Select: Use $\cM_{\rho'}$ to choose $m$ queries $\{q_{t,i} \}_{i\in[m]} \subset Q$  and  set $Q_{t}\leftarrow Q_{t-1} \cup \{q_{t,i} \}_{i\in[m]}$. 
    \sa{Selection criteria is not clear}\gv{This was intentional but we can make it more concrete. }
    \State 2) Measure: Add Gaussian noise $\hat{a}_{t,i} = q_{t,i}(D) + \eta$ where $\eta\sim \cN(0, \tfrac{1}{\rho'})$ for each $i\in[m]$. 
    \sa{Add for each i? Also $a$ should be $\hat{a}$, right? $\rho'$ is not defined.}
    %
    \State 3) Projection Step: Let $\hat{a}_{t} \in \mathbb{R}^{m \cdot t}$ be the noisy answers to all queries in $Q_t$. And let $q_{t}:\cX\rightarrow \mathbb{R}^{m \cdot t}$ be query function that answers all queries in $Q_{t}$. Then use an \textit{optimization oracle} to solve the following objective: 
    \begin{align*}
        D_{t}^{'}\leftarrow \argmin_{D'} \| \hat{a}_t - q_t(D') \|_2
    \end{align*}
\EndFor

\State \textbf{Output:} $D_{T}^{'}$
\end{algorithmic}
\end{algorithm}

==> docs/algos/rap_pp.tex <==
\begin{algorithm}
\caption{\rappp }\label{alg:rappp}
\begin{algorithmic}[1]
\Require A Dataset $D$. 
\State Instantiate \cref{alg:framework} with query set $Q $, where $Q$ consist of all 1 and 2-way marginal queries (\cref{def:mixed}), a discrete set of  1 and 2-way prefix queries ( \cref{def:thresqueries}), and a discrete set of mixed-marginal queries (\cref{def:mixed}).

\State And the Report Noisy max algorithm with score function $f:Q \times \hat{\cX}^{n'} \rightarrow [0,1]$, defined as 
\begin{align*}
f(q, D') = \|q(D) - q(D') \|_2
\end{align*}
\end{algorithmic}
\end{algorithm}

==> docs/checklist.tex <==
\section*{Checklist}


% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} We currently focus on providing private synthetic data for downstream ML tasks with linear models. 
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} 
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{} 
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
    
    The ACS dataset was released by the US Census Bureau publicly, and we follow the terms of service of the ACS data in our use. The terms of service can be found here: \href{https://www.census.gov/data/developers/about/terms-of-service.html}{https://www.census.gov/data/developers/about/terms-of-service.html}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} 
    
    According to the Terms of Service (\href{https://www.census.gov/data/developers/about/terms-of-service.html}{https://www.census.gov/data/developers/about/terms-of-service.html}) of the ACS data, "The Census Bureau has created these data to exclude information that would directly identify respondents and characteristics that may lead to the identification of respondents." and "... users will not use these data, alone or in combination with any other Census or non-Census data, to identify any individual person, household, business or other entity; not link or combine these data with information in any other Census or non-Census dataset in a manner that identifies an individual person, household, business or other entity; not publish information from these data files, particularly in combination with any other Census or non-Census data, in a manner that identifies any individual person, household, business or other entity; and not use the identity of any person or establishment discovered inadvertently ..." We follow the Terms of Service in our use of the ACS data.
    
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}



==> docs/figures/acs_singletask_summary.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/acs/acs(single task) summary.png}
    \caption{Performance difference summary of \cref{fig:acsml}
    . }
    \label{fig:acsml}
\end{figure}

==> docs/figures/datasets.tex <==
% \begin{table}[]
%     \centering
%     \begin{tabular}{||c|c|c|c||}
%     \hline
%          Dataset name & Rows & Numerical & Categorical \\
%     \hline
%     Generated high dimensional & 16000& d & 1 \\ 
%     \hline
%     Generated Low Information Generated  & 16000 & d & 1 \\ 
%     \hline
%     ACS NY (Income)  & 100513 & 4 & 6 \\ 
%     \hline
%     ACS CA  (Income) & 183941 & 4 & 6 \\ 
%     \hline
%     ACS TX  (Income) & 127039 & 4 & 6 \\ 
%     \hline
%     ACS PA  (Income) & 66540 & 4 & 6 \\ 
%     \hline
%     ACS FL  (Income) & 66540 & 4 & 6 \\ 
%     \hline
%     \end{tabular}
%     \caption{Dataset descriptions.}
%     \label{tab:datasets}
% \end{table}

==> docs/figures/multi/data_desc.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
         State & Rows & Categorical & Numerical & OH-Dimension   \\
    \hline
    \hline
    NY & 196276 & 25 & 9 & 151 \\ 
    \hline
    CA & 372553 & 25 & 9 & 151\\ 
    \hline
    TX & 254883 & 25 & 9 & 151 \\ 
        \hline
    FL & 192673 & 25 & 9 & 151 \\ 
    \hline
    PA & 127859  & 25 & 9 & 151 
    \end{tabular}
    \caption{Multi Target ACS descriptions.\gv{Replace this with a footnote.}}
    \label{tab:multidataset}
\end{table}

==> docs/figures/multi/ml_summary.tex <==
\begin{figure}
    \centering
    \textbf{Summary of ACS Multi Task ML}\par\medskip
    \includegraphics[width=\textwidth]{docs/figures/multi/ml_summary_multi.png}
    \caption{Machine learning F1 score summary over all states.
     \gv{Missing old-RAP} 
    %  \ar{What does summary mean? Average over states?} \ar{In the individual state breakouts, we seem to beat PGM on each state in travel, but they do better in the summary? What is going on? }
    }
    \label{fig:acsml}
\end{figure}

==> docs/figures/runtime/runtime_vs_f1_ALL.tex <==

% Shuai you can make this smaller. make the width 0.5
\begin{figure}{l}
% \begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{docs/figures/runtime/runtime_vs_f1_all_tasks_NY.png}
    \caption{
    % \gv{Placeholder. Need to fix legend and add markers for different bin sizes. }
    \textbf{F1 score vs. Runtime .}
   Comparing \rappp (blue) and PGM (orange) for different hyperparameter choices over five ACS single-task datasets and $\epsilon=\{0.15, 1\}$. 
   PGM parameter bin-size is varied by selecting from $\{10, 20, 50, 100\}$. \rappp parameter for the number of  epochs for linear thresholds ($T_{LT}$) is varied by selecting from $\{10, 30, 50, 70\}$.
   % 
    %
    % All results are for NY state. 
    % \rappp runtime is faster than \pgm. Having more columns in a task leads to drastic increase of runtime for \pgm, but the runtime of our \rappp is consistent across tasks, and only varies a little when more random linear queries are computed. Furthermore, \rappp's f1 score is relatively consistent across different hyperparamter choices whereas the \pgm's f1 score is sensitive to the choice of bin size. 
    }
    \label{fig:runtime}
    % \end{figure}
\end{figure}



% We can wrap this

==> docs/figures/runtime/runtime_vs_f1_all_tasks_NY.tex <==

% % Shuai you can make this smaller. make the width 0.5
% \begin{wrapfigure}{l}{1.0\textwidth}
% % \begin{figure}
%     \centering
%     \includegraphics[width=1\textwidth]{docs/figures/runtime/runtime_vs_f1_all_tasks_NY.png}
%     \caption{
%     % \gv{Placeholder. Need to fix legend and add markers for different bin sizes. }
%     \textbf{F1 score vs. Runtime .}
%   Comparing \rappp (blue) and PGM (orange) for different hyperparameter choices over five ACS single-task datasets and $\epsilon=\{0.15, 1\}$. 
%   PGM parameter bin-size is varied by selecting from $\{10, 20, 50, 100\}$. \rappp parameter for the number of  epochs for linear thresholds ($T_{LT}$) is varied by selecting from $\{10, 30, 50, 70\}$.
%   % 
%     %
%     % All results are for NY state. 
%     % \rappp runtime is faster than \pgm. Having more columns in a task leads to drastic increase of runtime for \pgm, but the runtime of our \rappp is consistent across tasks, and only varies a little when more random linear queries are computed. Furthermore, \rappp's f1 score is relatively consistent across different hyperparamter choices whereas the \pgm's f1 score is sensitive to the choice of bin size. 
%     }
%     \label{fig:runtime}
%     % \end{figure}
% \end{wrapfigure}



% % We can wrap this

==> docs/figures/sigmoid_plot/sigmmoid_neurips.tex <==


% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{docs/figures/sigmoid_plot/sigmoid_optimization_CA.png}
%     \caption{
%     \gv{Show only one state.}
%     % Comparing naive Sigmoid optimization vs Sigmoid annealing.\gv{Move legend to top.}
%     Comparing the max and average error of the Sigmoid temperature Annealing technique from \cref{alg:oracle} against fixed-sigmoid optimization.   The underlying dataset is multitarget ACS, described in \cref{sec:experiments},\ar{Should have a pointer to where this is described since the reader doesn't know at this point what this is}\gv{Added this} on 5 different states and the error is over a set of $1000$ random $2$-way mixed-marginal queries (see \cref{def:mixed}).
%   % 
%     The blue curve represents the error after fixing the Sigmoid parameter for  Sigmoid values in the set $\{2^1\ldots, 2^{15}\}$.
%     The x-axis gives the value of the Sigmoid parameter and the $y$-axis is the error. 
%   % 
%     For each Sigmoid parameter we report the average max and mean error over 10 runs of the algorithm with $95$ percent confidence intervals.   
%   % 
%   Finally, 
%     the red dashed horizontal line is the average error over 10 runs  after using Sigmoid temperature annealing in the optimization.
%   %  
%     }
%     \label{fig:annealing}
% \end{figure}
 
 \begin{wrapfigure}[18]{r}{0.45\textwidth}
  \begin{centering}
   \includegraphics[trim=0mm 0mm 0mm 5mm, width=0.40\textwidth, clip]{docs/figures/sigmoid_plot/sigmoid_optimization_CA.png}
  \end{centering}
  \caption{ \small 
  Comparison of the Maximum error (left) and the Mean error (right) of optimizing mixed marginals using our temperature annealing (red line) and using a fixed $\sigma$ parameter (blue curve). It is clear that annealing the $\sigma$ parameter strategically during optimization leads to lower error than using any fixed $\sigma$ parameter during the continuous projection step.
%   Comparison of temperature annealing (red line) with sigmoid with a fixed parameter (blue curve) in terms of approximation errors. 
%   Left: Maximum error, Right: Mean error.
%   Comparing naive Sigmoid optimization vs Dynamic Sigmoid Scaling \ar{Haven't seen this name elsewhere}. 
The error is over a set of $1000$ random $2$-way mixed-marginal queries (see \cref{def:mixed}). And the underlying dataset is described in detail in \cref{sec:experiments}.
%   The x-axis gives the value of the Sigmoid parameter and the $y$-axis is the error. 
%   The blue curve represents the error of fixing the Sigmoid parameter for values in the set $\{2^1\ldots, 2^{15}\}$. Finally, 
%     the red dashed horizontal line is the average error over 10 runs  of  the sigmoid temperature technique. See appendix for results on other datasets.
  }
  \label{fig:annealing}
\end{wrapfigure}

==> docs/figures/single/summary.tex <==
\begin{figure}
    \centering
    \textbf{Summary of ACS Single Task ML}\par\medskip
    \includegraphics[width=\textwidth]{docs/figures/single/ml_summary_single.png}
    \caption{Machine learning F1 score summary over all states.
     \gv{Missing old-RAP} \gv{Describe how we choose the best parameter for PGM.}
    %  \ar{What does summary mean? Average over states?} \ar{In the individual state breakouts, we seem to beat PGM on each state in travel, but they do better in the summary? What is going on? }
    }
    \label{fig:acsml}
\end{figure}

==> docs/old/Approach.tex <==
\section{RAP++ with Continuous Approximation}
We build on the Relaxed Adaptive Projection algorithm from \cite{aydore2021differentially}.
At a high level, the original RAP algorithm obtains noisy measurements using the Gaussian Mechanism, where the noisy measurements are denoted by $\widehat{a} = q(D) + \cN(0, \sigma^2)$, and then projects a synthetic dataset $\widehat{D}$ to fit the noisy measurements. If $D$ be the real dataset,  $q:\cX^{n} \rightarrow \mathbb{R}^m $  is a function that gives the answer to all $m$ queries on any input dataset, then the optimization project that RAP is trying to solve is
%
%
\begin{align}\label{eq:obj}
    \min_{\widehat{D} \in \cX^{n'}} \| \widehat{a} - q(\widehat{D}) \|
\end{align}

Solving the problem \eqref{eq:obj} is computationally hard, therefore the original RAP algorithm uses an optimization procedure based on gradient descent.
That is, to find $\widehat{D}$, RAP first initializes a random dataset $\widehat{D}_0$ and then applies gradient descent on $\widehat{D}_0$ until the error is small.  In short, their algorithm works as follows:
\begin{itemize}
    \item Initialize a synthetic dataset $\widehat{D}$ in some domain $\cX$ where the true dataset $D$ lies. Extend $\cX^{\text{cat}}$ to continuous space by one-hot-encoding and allowing values between 0 and 1 for each entry.
    \item Privately select a subset of queries $Q'\subset Q$ {\it differentiable queries} where the answers on $D$ and $\widehat{D}$ differ the most, and privately compute their answers on $\widehat{D}$.
    \item Given a subset of $m'$ differentiable queries $q':\cX^*\rightarrow[0,1]^{m'}$ and measurements $\hat{a}' = q'(D) + \cN(0, \sigma^2)$, use gradient-based optimization on  $\widehat{D}$ to optimize equation \eqref{eq:obj}.
    % using the difference from $D$ on the selected queries as the loss function.
    \item Continue iteratively selecting and preserving more queries until the privacy budget is exhausted.
\end{itemize}

To summarize, RAP requires that the objective \eqref{eq:obj} is differentiable and to make the objective differentiable RAP relaxes the data domain to be continuous.
Then the marginal queries can become differentiable queries.

A {\it differentiable query} is a statistical query (the average value of a function over the rows of $D$) which is represented by a differentiable function. This can always be done for queries over boolean data, e.g.\ by polynomial interpolation. We refer to each update of the query set (and subsequently, $\widehat{D}$) as an {\it epoch}.



However, interval queries are step functions on continuous features, which are not differentiable. Therefore, in this work we propose using smooth functions to approximate the interval queries. Suppose that in our optimization problem (equation \eqref{eq:obj}), the function $q:[0,1]\rightarrow \{0,1\}^m$ represents the answers to a set of interval queries. The main idea behind RAP++ is to approximate $q$ with a smooth function $\widetilde{q}:[0,1]\rightarrow [0,1]^m$ which we can take gradients over. We choose Sigmoid functions as our approximating functions because it has nice gradients and it allows us to control the approximation error.

\begin{definition}[Sigmoid function.]\label{def:sigmoid}
% Let $f_a:[0,1]\rightarrow \{0,1\}$ be a threshold function with threshold $a\in[0,1]$. 
The sigmoid threshold function $s_{a,\sigma}:[0,1]\rightarrow [0,1]$ with threshold $a\in[0,1]$ and parameter $\sigma>0$   is defined as $s_{a,\sigma} = \left(\frac{1}{1+e^{-\sigma(x-a)}}\right)$  for any $x\in[0,1]$.
\end{definition}


The sigmoid function is a differentiable approximation of the class of threshold functions.
The parameter $b>0$, in definition \ref{def:sigmoid}, controls the approximation error of the sigmoid function, where larger $b$ gives better approximation to the corresponding threshold function. 
% threshold function $f_a:[0,1]\rightarrow \{0,1\}$  with threshold $a\in[0,1]$, we have $\lim_{b\rightarrow \infty} \sigma_{a,b}(x) = f_a(x) $ for all $x\in [0,1]$. 
Once we have a  differentiable function we can use RAP to answer the interval queries. However there are three challenges that arise when we the sigmoid approximation: Flat gradients/diminishing gradients and boundary conditions. 

The sigmoid function over the real line can suffer from flat regions which leads to very small gradients. In the flat gradient regime it's possible that the gradient optimization becomes stuck. One solution is to randomly initialize multiple interval queries over the continuous domain to minimize the chance that the variable points will appear in flat areas. A second issue we encountered is boundary conditions, that is if much of the data is too close to the threshold of any threshold, then the sigmoid function for that threshold will give a bad approximation. The solution again is randomization, we sampling random intervals you reduced the change that all the points will be concentrated near any one threshold. 




==> docs/old/algorithm.tex <==
\section{Algorithm}

In this section, let $q$ be the query function that computes the answers for $m$ queries. For any dataset $D$, the noisy target answer vector with noise is denoted by $\hat{a} = q(D) + \eta$, where $\eta\in \mathbb{R}^m$ is a random noise vector sample from the Gaussian distribution. 
Our goal is to find a synthetic dataset $D'$ such that  the error $ \| \widehat{a} - q(\widehat{D}) \|$ is minimized. This terms is difficult to optimize, but as shown in \cite{aydore2021differentially} we may use a continuous representation of the queries and apply gradient descent techniques.
%
%
In this paper we used the Sigmoid funciton

Therefore, if we let $\tilde{q}_{\sigma}$ be the continuous Sigmoid approximation of $q$ with parameter $\sigma\in \mathbb{R}^m$ \gv{(TODO: formally define $\sigma$)}, then  we can upper bound the error term with the following decomposition: 
%
%
%
\begin{align}\label{eq:objupperbound}
    \| \widehat{a} - q(\widehat{D}) \|
    \leq  \underbrace{\| \widehat{a} - \tilde{q}_\sigma({D'}) \|}_{\text{noisy statistic error}} +  \underbrace{\| q({D'}) - \tilde{q}_\sigma({D'})\|}_{\text{approximation error}}
\end{align}
%

The first term of \eqref{eq:objupperbound} is the noisy statistics error of the synthetic dataset $D'$ by using the continuous queries. And the second term represents the approximation error of the continuous queries when evaluated on $D'$. The basic idea is to simultaneously optimize both term by means of gradient descent. This is possible because the both terms are continuous functions of the optimization variables $D'$ and $\sigma$.
% Given a set of queries and a dataset main algorithm \ref{alg:rpppl}, first computes the answers to all the queries, which we denote with the vector $\hat{a}\in\mathbb{R}^m$ and then finds a synthetic dataset thjat 


\paragraph{Solution} The solu



\begin{algorithm}
\caption{Relaxed-Projection-with-Sigmoid-Adaptivity (Similar to \cite{aydore2021differentially})}\label{alg:rp}
\begin{algorithmic}
\Require Learning rate parameters $\alpha$ and $\gamma$, number of interations $T$.

% and continuous approximation parameters $\sigma_1$, $\gamma$. 
\State \textbf{Input} A query function $q: \cX^r \rightarrow \mathbb{R}^m$, a vector of target answers $\hat{a} \in \mathbb{R}^m$, and an initial dataset $D_1'$ and initial Sigmoid parameter $\sigma_1$.


\For{$t =1$ \textbf{to} $T$}
    \State  Gradient Descent: 
    $$D'_{t+1} \leftarrow  D_t' - \alpha \nabla_{D'_t} \|\hat{a} - \tilde{q}_{\sigma_t}(D'_t) \|   
    \quad \quad \text{and } \quad 
    \quad \sigma_{t+1} \leftarrow  \sigma_t - \gamma \nabla_{\sigma_t} \|q(D'_{t+1}) - \tilde{q}_{\sigma_t}(D'_{t+1}) \| $$\;
    % \State Set $\sigma_{t+1}$ to decrease $\| q({D_{t+1}'}) - \tilde{q}_{\sigma_t}({D_{t+1}'})\|$ with rate $\gamma$
    % \State Set  $L_{t+1} \leftarrow \|\hat{a} - \tilde{q}_{\sigma_t}(D'_{t+1}) \| + \| q({D_{t+1}'}) - \tilde{q}_{\sigma_t}({D_{t+1}'})\|$
    % \If{$|L_t - L_{t-1}| < \text{stopping-threshold}$}
    %     \State Halt and output $D_{t+1}'$
    % \EndIf
\EndFor
%
\State \textbf{Output:} $D_T'$
\end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Main Algorithm
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{algorithm}
\caption{RAP++}\label{alg:rppp}
\begin{algorithmic}
\Require  A learning rate parameter $\alpha>0$, optimization rounds $T$.
\State \textbf{Input} A dataset $D$ with $n$ records, a collection of $m$ statistical queries $Q$, the size of the synthetic dataset $n'$, and differential privacy parameters $\varepsilon, \delta$.
\State Let $\rho$ by such that: 
\begin{align*}
    \varepsilon = \rho + 2\sqrt{\rho \log(1/\delta)} 
\end{align*}

\State Let $q:\cX^n \rightarrow \mathbb{R}^m$ be the function that computes all the answers in $Q$.
\State Evaluate query answers using the Gaussian mechanism: Let $\hat{a} = q(D) + Z$, with  $Z \sim \mathcal{N}\left(0, \frac{1}{2n^2 \rho}\right)$.
% \State Initialize the Sigmoid vector $\sigma_1\in \mathbb{R}^m$ and the sigmoid update rate $\gamma$. 
%
\State Initialize $D'_1\in \cX^{n'}$ and $\sigma_1 \in \mathbb{R}^m$.
\State Project step: $D' \leftarrow \text{Relaxed-Projection}(\tilde{q}, \hat{a}, D'_1, \sigma_1, \alpha, \gamma)$ 
    % \State Set $D'_{\text{best}}$ to $D'$ if $D'$ has lower error.
% \State $D'_{\text{best}} \in \argmin \{ D_{\sigma, \gamma} \}$.
\State \textbf{Output:} $D'$
\end{algorithmic}
\end{algorithm}

==> docs/old/analysis.tex <==
\section{Analysis of Sigmoid Continous Approximation Error}

% In this section we analyze the continuous approximation worst case guarantees. We begin by giving a negative result about the worst case error of the Sigmoid approximation.

In the previous section we showed how to  

In this section we denote a set of query statistics as $Q$ and any single query as $q\in Q$. We consider threshold statistics only as in \cref{def:thresqueries} and for any threshold query $q\in Q$ we say that its continuous approximation is $\tilde{q}$. Furthermore, given a set of statistics $Q$ and any dataset $D$ the surrogate error of a synthetic dataset $D'$ on query $q$ is given by $|\tilde{q}(D) - \tilde{q}(D')|$ and its real error is $|q(D) - q(D')|$.
 
%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposition 1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{propositionrep}\label{thm:singlequeryerror} Let $q:[0,1]^n\rightarrow [0,1]$ be a $1$-way threshold statistic and let $\tilde{q}$ be its continuous approximation. Then there exist datasets $D$ and $D'$
, such that $\left| \tilde{q}(D) - \tilde{q}(D')\right| = 0$ and $\left| {q}(D) - {q}(D')\right| \geq 0.5$.
\end{propositionrep}
\begin{proof}
Let $q$ be a non-trivial threshold function defined as $q(x) = \mathbb{I}\{x>=0.5\}$. Then let $D' = \{0.4999 \}_{i=1}^n$ by a dataset with $n$ rows each with value $0.4999$. Then we have that $q(D') = 0$ and $\tilde{q}(D') \approx 0.5$. Therefore the approximation error is $|q(D')-\tilde{q}(D')| \approx 0.5$
\end{proof}
%
%
The \cref{thm:singlequeryerror} says that for any threshold query $q$ we can always find a pair of datasets such that the surrogate error (i.e., $|\tilde{q}(D)-\tilde{q}(D')|$) is  small but the real error (i.e., $|q(D)-q(D')|$) is large. However, we usually optimize a large number of threshold queries simultaneously. For the next results we assume we have access to an optimization oracle that finds the optimal solution to a large set of threshold queries, we give the definition here:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{definition}[Continuous approximation Oracle]\label{def:oracle}
%  For any query $q$ we denote its continuous approximation as $\tilde{q}$. Then given a set of threshold statistics $Q$, and a dataset $D$, a continuous approximation oracle finds a dataset $D'$ such that
% %
% \begin{align*}
%   \max_{q\in Q} \left| \tilde{q}(D) - \tilde{q}(D')\right| = 0
% \end{align*}
% \end{definition}
%
% The next result says that even when we perfectly optimize the surrogate loss of a large number of threshold queries, then the worst case lower bound of \cref{thm:singlequeryerror} still applies.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposition 2
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{propositionrep}\label{thm:oraclemax}
% Given a set $Q$ threshold statistics, there exist a dataset $D$ such that a continuous approximation oracle (as in \cref{def:oracle}) finds  a dataset $D'$ with $\max_{q\in Q} \left| \tilde{q}(D) - \tilde{q}(D')\right| = 0$, however 
% $\max_{q\in Q}\left| {q}(D) - {q}(D')\right| \geq 0.5$.
% \end{propositionrep}


% Unfortunately, \cref{thm:oraclemax} shows that on any single query we cannot guarantee a good approximation of a threshold statistics when using a continuous surrogate. The reason is that we can always find a dataset that puts all the points very near the threshold of the query, which would always evaluate to 0.5 on the  approximation but can take  value  $0$ or $1$ on the real threshold function. However, if in the set of statistics is diverse enough then we can at least say that the average approximation error over all the threshold queries has to be small. The next results gives an average case guarantee. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Proposition 3
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{propositionrep}\label{thm:averageQ} Let 
% $Q_{m}=\{q_k \}_{k=1}^m$ be a set of $m$ threshold statistics, where for any $k\in[m]$ the corresponding query $q_{k}$ is defined as 
% $q_{k}(x) = \mathbb{I}\{x< \frac{k}{m}\}$ on all $x\in[0,1]$. And let $\tilde{q}_k$ be the continuous Sigmoid approximation of query $q_k$, defined as $\tilde{q}_k(x) = \left(1 + \exp(-\sigma(x - {k}/{m}))\right)^{-1}$ on all $x\in[0,1]$, where $\sigma>0$ is the Sigmoid function parameter.

% For all datasets $D\in[0,1]^n$, if $\sigma = \sigma(m)$ and assuming we have access to an oracle that finds a solution  $D'$ such that  $\max_{k\in[m]} \pp{\tilde{q}_k(D) - \tilde{q}_k(D')} = 0$. Then we have that 
% \begin{align*}
%   \frac{1}{m} \sum_{k=1}^m \left( q_k(D) - q_k(D') \right)^2 \leq C(m)
% \end{align*}
% where $C(m)$ is a small number that depends on $m$.
% \end{propositionrep}
% \begin{proof}

% We begin by given a result that hold for the class of evenly spread out threshold queries. Let $Q_{m} = \{q_{\frac{k}{m}}:  [0,1] \rightarrow \{0,1\} | k \in [m] \}$ be the class of $m$ prefix queries where each $q_{\frac{k}{m}}$ is defined as in \cref{def:thresqueries}. Let us restate the definition here: For any $k\in[m]$ and any $x\in[0,1]$, we have $q_{\frac{k}{m}}(x) = \mathbb{I}\{x< \frac{k}{m}\}$. Note that the prefix queries in $Q_m$ are evenly spread out in the range $[0,1]$.


% For simplicity, we consider only datasets with only one continuous column with range $[0,1]$. We denote the class of datasets with $n$ rows and a single continuous feature as  $\cD^n = [0,1]^n$.

% Our goal is to bound the approximation error, which is defined as:
% %
% \begin{align}\label{eq:approxerror}
%      \max_{D\in [0,1]^n} \frac{1}{m} \sum_{q\in Q_{m}} \left( q(D) - \tilde{q}(D) \right)^2
% \end{align}

% The first step is to show the worst average approximation error error happens when $D$ puts all its mass very near the threshold of some prefix query. Show that 

% \begin{align}\label{eq:worstcaseinequality}
%     \max_{D\in [0,1]^n} \frac{1}{m} \sum_{q\in Q_{m}} \left( q(D) - \tilde{q}(D) \right)^2
%     \leq \max_{x\in [0,1]} \frac{1}{m} \sum_{q\in Q_{m}} \left( q(x) - \tilde{q}(x) \right)^2
% \end{align}
 
% TODO: Complete proof of \cref{eq:worstcaseinequality}. 

% Then, we can show for any fixed $x\in [0,1]$
% \begin{align*}
%     &\frac{1}{m}\sum_{k=1 }^{m} \left(q_{k}(x) - \tilde{q}_{k}(x) \right)^2  \\
%     % %
%     &= \frac{1}{m}
%     \left[
%         \sum_{k=1}^{m x} \left(1 - \tilde{q}_{k}(x) \right)^2 
%         + \sum_{k=m x+1}^{m} \left(- \tilde{q}_{k}(x) \right)^2 
%     \right]
%         && (\text{if } k < mx \text{ then } q_k(x) = 1)  \\ 
%     %
%     &= \frac{1}{m}
%     \left[
%         \sum_{k=1}^{m x} 
%         \left(
%             1 - \frac{1}{1 + \exp\pp{-\sigma (x-\tfrac{k}{m})}}
%         \right)^2 
%         + 
%          \sum_{k=m x+1}^{m} 
%         \left(
%             - \frac{1}{1 + \exp\pp{-\sigma (x-\tfrac{k}{m})}}
%         \right)^2 
%     \right] 
%     && (\text{if } k < mx \text{ then } q_k(x) = 1)
% \end{align*}

% First we bound the term $\sum_{k=m x+1}^{m} \frac{1}{\left(1+\exp\pp{-\frac{x k  \sigma}{m}}\right)^2}$. For any $x\in[0,1]$ we have
% %
% %
% \begin{align*}
% &\sum_{k=m x+1}^{m} 
%       \frac{1}{m} \left(
%             - \frac{1}{1 + \exp\pp{-\sigma (x-\tfrac{k}{m})}}
%         \right)^2 \\  
% %
% %
% &\leq \int_{k=m x+1}^{m} \frac{1}{\pp{1 + \exp\pp{-\sigma (x-\tfrac{k}{m})}}^2} dk\\
% %
% %
% &= \int_{k=m x+1}^{m} \frac{1}{\pp{1 + \exp\pp{-\sigma x}\exp\pp{\sigma\tfrac{k}{m})}}^2}dk \\
% %
% %
% &=
%  \left[
%  \frac{m\pp{
%  \frac{1}{\exp\pp{k\sigma / m} + 1}
%  -
%  \log\pp{\exp\pp{k\sigma/m} + \exp\pp{\sigma x }}
%  }}
%  {\sigma} + k 
%  \right]_{mx +1}^m
% %
% %
% %
% % &= 
% % \bb{
% % k  - \frac{m\log\pp{\exp\pp{(k\sigma)/m} + \exp\pp{\sigma x}}}{\sigma}
% % }_{mx +1}^m\\
% % %
% % %
% % &=\bb{m - \frac{m\log\pp{\exp\pp{(m\sigma)/m} + \exp\pp{\sigma x}}}{\sigma}}
% % -
% % (mx + 1)  + \frac{m\log\pp{\exp\pp{((mx+1)\sigma)/m} + \exp\pp{\sigma x}}}{\sigma}\\
% % %
% % %
% % &= m(1-x) - 1 + 
% % \frac{
% %     -m\log\pp{\exp\pp{(m\sigma)/m}} + m\log\pp{\exp\pp{((mx+1)\sigma)/m}}
% % }{\sigma}
% \end{align*}

% \end{proof}



\begin{propositionrep}
For any privacy parameter $\varepsilon, \delta$, a synthetic data size $n'$ and any set of $m$ $k$-way mixed marginal queries. If the optimization in the projection step is solved exactly, then the RAP++ mechanism outputs a synthetic dataset $D'$ with average error bounded as:
\begin{align*}
    \sqrt{\tfrac{1}{m}\|q(D) - q(D')\|_2^2}
    \leq  O
 \left( 
 \frac{d'(\log{k} + \log{n'}) + \log(1/\beta)(\ln(1/\delta))^{1/4}}{\sqrt{\varepsilon n}}
 +\frac{\log(k)}{\log(n')}
 \right) 
 + \sqrt{\tfrac{1}{m}\|q(D) - \tilde{q}_\sigma(D')\|_2^2}
\end{align*}
\end{propositionrep}
\begin{proof}
Assume that the optimization finds a dataset $D'$ and a sigmoid parameter $\sigma$ such that 
$\|\hat{a} - \tilde{q}_\sigma(D')\|_2  = 0$. 
Then we can apply Theorem 4.1 in as follows:

\begin{align*}
    &\tfrac{1}{m}\|q(D) - q(D')\|_2^2 \\
    &\leq \tfrac{1}{m}\|q(D) - \tilde{q}_\sigma(D')\|_2^2 + 
    \tfrac{1}{m}\|q(D') - \tilde{q}_\sigma(D')\|_2^2 \\
&\leq 
    \left[
     O
     \left( 
     \frac{d'(\log{k} + \log{n'}) + \log(1/\beta)(\ln(1/\delta))^{1/4}}{\sqrt{\varepsilon n}}
     +\frac{\log(k)}{\log(n')}
     \right) 
     \right]^2
     + \tfrac{1}{m}\|q(D') - \tilde{q}_\sigma(D')\|_2^2 \\ 
\end{align*}
\end{proof}

==> docs/planning/timeline.tex <==



\section{Timeline}
\begin{enumerate}
    \item \textbf{March 15}:\sout{ Finish ML experiments for RAP and PGM, including datasets:}
        \begin{enumerate}
        \item ADULT, ACS-NY, shopping, classification-5d dataset.
    \end{enumerate}
     \item \textbf{March 15}: \sout{Write down  optimization algorithm for Sigmoid queries}. Highlight Key technique which is to use a dynamic Sigmoid parameter.
    \item \textbf{March 22}: Scale RAP++:
    \begin{enumerate}
        \item \sout{Compare projection algorithm with and without heuristics. Remove base error from bar plot in\cref{fig:oracletest}. }
        \item \sout{Optimize RAP++ to run on larger datasets.}
        \item \sout{Grid search to search a the combination of hyperparameters for RAP++ that do better on the Adult dataset. }
        \item \sout{Run RAP++ on ACS.}
        \item \sout{Run RAP++ on Shopping.}
        \item \sout{Run RAP++ on Circles from sklearn.}
        \item \sout{Figure out what the bars mean in the plots.}
    \end{enumerate}
    \item \textbf{March 22}: Experiment Section First Draft: 
    \begin{enumerate}
        \item Include description of datasets used.
        \item Describe RAP, PGM, GEM.
        \item Describe ML experiments setup.
    \end{enumerate}
    \item \textbf{March 30}: High dimensional continuous Data Experiments.
    \begin{enumerate}
        \item Run Experiments on \textit{Classification-50d}. This toy dataset has 50 continuous features, which is much larger than anything tried before. We already see that both PGM and RAP do not perform well on low dimensional continuous data. \sout{Therefore, we want to see how PGM and RAP do against 50 continuous columns in terms of Machine learning.}\gv{PGM fails to run on Classification-50d for epsilon 0.1 or higher.}
        \item Run RAP++  on classification-50d: The resulting number of queries for this dataset will be very large and will result in RAP++(with prefix queries) to run very slow. An alternative approach is to run RAP++ with halfspace queries. 
    \end{enumerate}
    
    \item \textbf{April 4}:
    \begin{enumerate}   
        \item  DP-MERF baseline using our own implementation.
        \item Implement GEM and run experiments.
        \item RAP++ with Prefix Queries on Fourier features.
    \end{enumerate}
\end{enumerate}

==> docs/planning/todo.tex <==



\section{Tasks}


\begin{itemize}
    \item Open questions:
    \begin{enumerate}
        \item What types of queries do we want to preserve? 
        \item What is the Optimization Algorithm for threshold queries? 
        \item What data features do we need to preserve for Machine Learning?
    \end{enumerate}
    \item Run the following algorithms:
        \begin{enumerate}
        \item RAP++ Using Random Linear Features and Threshold queries. 
        \item Use a generative model (i.e., GEM++) plus  Random Linear Features with threshold queries. 
        \item RAP and Private-PGM as benchmark for tabular data. Both  these algorithms  discretize continuous features into 100 bins. 
        \item DP-MERF and DP-GANs as benchmark for \textit{image} data.
        \item PRIVATE POST-GAN BOOSTING
    \end{enumerate}
    
    \item datasets:
    \begin{enumerate}
        \item Tabular data: Adult and  ACS (NY, FL, PA, ...) (and other datasets listed in \cite{tao2021benchmarking}).
        \item Image data: MNIST and Fashion-MNIST.
    \end{enumerate}


    
    \item Metrics to compare:
    \begin{enumerate}
        \item 1 and 2-way mixed marginal queries. If we preserve 1 and 2-way marginal queries, how well do we generalize to higher $k$?
        \item binary classification accuracy using linear models and XGBoost classifier.
        \item Multi-task/multiclass classification accuracy using XGBoost.
    \end{enumerate}
    
    \item Describe RAP with sensitivity trick and new oversampling technique.
    \item Describe PGM and why we use it as as benchmark.
    
\end{itemize}

\input{docs/timeline}

==> docs/relaxed.tex <==
\section{Relaxed Projection with Threshold Queries}\label{sec:relaxed}
% \section{Efficient Optimization Oracle for Threshold Queries.}
% Goal for this section.
% \begin{enumerate}
%     \item  Explain why the optimization problem in \cref{eq:objectivediff} is hard independent of Differential Privacy and enumerate the challenges.
%     \item Explain the heuristics that we have develop to tackle this problem.
%     \item Prove that we solved this problem with empirical evidence. Design interesting experiments.
% \end{enumerate}
% In order to implement the projection step in \cref{alg:framework}

% \gvdelete{
% % In this section we propose a gradient-based optimization algorithm for learning a numerical synthetic dataset that approximates the answers to threshold based queries over continuous data
% . %, as defined in \cref{def:prefix}, \cref{def:mixed} and \cref{def:linearthreshold}, given that we have access to their noisy answers. 
% %
% Our algorithm \mk{More naming confusion. Is this what earlier we were calling tempered/temperature, which I complained about above? And when it uses the term relaxed projection, and we call it ``our algorithm'', it makes it sound like the main RAPTOR algo rather than just a subroutine for one particular thing. Confusing.} "Relaxed Projection with Dynamic Sigmoid Scaling" is an extension of the \textit{relaxed projection} mechanism from \cite{aydore2021differentially} to linear threshold queries and mixed-type data.
% }


In this section we propose a gradient-based optimization routine  for learning a mixed-type synthetic datasets that approximate  answers to threshold based queries over continuous data.
The technique  is an extension of the \textit{relaxed projection} mechanism from \cite{aydore2021differentially}, which in turn  extends the \emph{projection mechanism} of  \cite{projection}.

%The projection mechanism consist of private measuring step where query answers are obtained using Gaussian mechanism. And a  

% Let us first describe the original 
 Given a dataset $D$, a collection of $m$ statistical queries $Q=\{q_1, \ldots, q_m \}$ and zCDP parameter $\rho$, the projection mechanism  \cite{projection} consists of two steps: (1) For each query index $i \in [m]$, evaluate $q_i$ on $D$ using the Gaussian mechanism: $\hat{a}_i = G(D, q_i, \rho/m)$, and then (2) Find a synthetic dataset $D'\in\cX^*$ whose query values minimize the distance to the noisy answers $\{\hat{a}_i\}_{i\in [m]}$: 
\begin{align}
\label{eq:objective}
    % \argmin_{D'\in \cX^{*}} \aveerror\pp{Q, D, D'}  
    \textstyle\argmin_{D'\in \cX^{*}} \sum_{i\in [m]} \left(\hat{a}_i - q_i({D}') \right)^2 .
    % \label{eqn:main_objective}  % Extra label
\end{align}
The projection step produces synthetic data that implicitly encodes the answers to all queries in the query set $Q$. In addition to producing synthetic data (which can be used for downstream tasks like machine learning which cannot easily be accomplished with the raw outputs of the Gaussian mechanism), by producing a synthetic dataset, the projection step by definition enforces consistency constraints across all query answers, which is accuracy improving.
Unfortunately, the projection 
step is generally an intractable computation since it is a minimization of a non-convex and non-differentiable objective over an exponentially large discrete space. %The first idea that goes into our algorithm is to 
To address this problem, \cite{aydore2021differentially} gives an algorithm that  relaxes the space of datasets $\cX^n$ to a continuous space, and generalizes the statistical queries to be differentiable over this space:

% \paragraph{Domain relaxation.}
\textbf{Domain relaxation.}
%Following \cite{aydore2021differentially}, our 
The first step is to represent categorical features as binary features using one-hot encoding. Let $d' \coloneqq  \sum_{i \in C} |\cX_i|$, where $C$ is the set of categorical features, be the dimension of the feature vector under the one-hot encoding. Then, we consider a continuous relaxation denoted by $\widetilde{\cX}$ of the  one-hot encoding feature space. Using $\Delta(\cX_i)$ to denote a probability space over the elements of $\cX_i$, we choose $\widetilde{\cX} \coloneqq \prod_{i\in C} \Delta(\cX_i)$ to be the product measure over probability distributions over the one-hot encodings. The advantage of representing the relaxed domain as a probability space is that one can quickly recover a dataset in the original discrete domain by random sampling.


% $\widetilde{\cX} = \prod_{i\in C} \Delta(\cX_i)$. 


% We further apply a SparseMax transformation to convert this relaxed data domain into the set of (sparse) probability distributions over one-hot encodings. This transformation allows us to apply randomized rounding to recover a dataset in the original schema. 


% \paragraph{Differentiable queries.}
\textbf{Differentiable queries.}
% The next step is to replace the set of queries $Q$  by a set of continuous and differentiable queries over the relaxed domain $\widetilde{\cX}$, which  we denote by $\widetilde{Q}$.
The next step is to replace the set of queries $Q$  by a set of continuous and differentiable queries $\widetilde{Q}$ over the relaxed domain $\widetilde{\cX}$.
% allows for  gradient based optimization.
% when the query set contains both marginal and threshold queries. 
% We show how to construct differentiable queries that approximate the original queries we care about.
% we replace the set of marginal and threshold queries by a set of differentiable queries over the relaxed domain.
%
Informally, in order to solve our optimization problem, the queries must be differentiable over the relaxed domain $\tilde{\cX}$ (and have informative gradients), but must also be a good approximation to the original queries in $Q$ so that optimizing for the values of the relaxed queries produces a synthetic dataset that is representative of the original queries. For categorical marginal  queries following \cite{aydore2021differentially}, we use the set of product queries over the relaxed domain which are %exactly 
equal to categorical marginal queries on the original domain: 
\begin{definition}
Given a subset of features  $T\subseteq [d']$ of the relaxed domain $\widetilde{\cX}$, the product query $q_T: \widetilde{\cX}$ is defined as $q_T(x) = \prod_{i\in T} x_i$.
\end{definition}

Next we give a differentiable relaxation for
any class of threshold based statistical queries such as those in \cref{def:mixed} and \cref{def:linearthreshold}.
% linear threshold queries
% \ar{And mixed/threshold marginals?}\gv{Saying we can handle any threshold based class.}
A linear threshold query is a threshold applied to a linear function of the data, which is not differentiable. We choose to approximate thresholds with sigmoid functions. They are a simple parametric class of functions with well-behaved gradients with adjustable magnitudes
% of the gradients %(important for optimization) 
for the approximation error via the \emph{inverse temperature} parameter:

\begin{definition}[Tempered Sigmoid]\label{def:sigmoid}
% Let $f_a:[0,1]\rightarrow \{0,1\}$ be a threshold function with threshold $a\in[0,1]$. 
The sigmoid threshold function $f^{[\sigma]}_{\tau}:\mathbb{R}\rightarrow [0,1]$ with threshold $\tau\in\mathbb{R}$ and inverse temperature  $\sigma>0$ is defined as $f^{[\sigma]}_{\tau}(x) = \left(\frac{1}{1+e^{-\sigma(x-\tau)}}\right)$  for any $x\in\mathbb{R}$.
\end{definition}




The sigmoid function in \cref{def:sigmoid} is a differentiable approximation of the class of $1$-way prefix marginal queries, which serves as a basic building block for approximating other interesting classes of threshold-based queries, 
% The parameter $b>0$, in definition \ref{def:sigmoid}, controls the approximation error of the sigmoid function, where larger $b$ gives better approximation to the corresponding threshold function. 
%The following definition uses sigmoid functions to approximate
such as the class of \emph{conditional linear threshold} queries.

\begin{definition}[Tempered Sigmoid Class Conditional Linear Threshold Queries]\label{def:sigmoidcond}
A {sigmoid conditional linear threshold query} is defined by a categorical feature $i\in[d']$ of the relaxed domain space, 
a set of numerical features $T\subseteq [d']$ in the relaxed domain space,
a vector $\theta\in\mathbb{R}^{|T|}$, and threshold $\tau\in \mathbb{R}$.
Fixing the sigmoid temperature $\sigma$, 
let $f_\tau^{[\sigma]}$ be defined as in \cref{def:sigmoid} then the corresponding differentiable statistical query is $    q^{[\sigma]}_{i, T, \theta, \tau}(x) = x_i \cdot f^{[\sigma]}_{\tau}(\dotp{\theta, x_T}) 
$.
% \begin{align*}
%     q^{[\sigma]}_{i, T, \theta, \tau}(x) = x_i \cdot f^{[\sigma]}_{\tau}(\dotp{\theta, x_T}) 
% \end{align*}
\end{definition}

By relaxing the data domain to its continuous representation $\widetilde{\cX}^{*}$ and replacing the query set $Q=\{q_1, \ldots, q_m\}$ by its differentiable counterpart $\widetilde{Q} = \{\tilde q_1,\ldots,\tilde q_m\}$ we obtain the new objective: 
\begin{align}\label{eq:objectivediff}
    % \argmin_{D'\in \cX^{*}} \aveerror\pp{Q, D, D'}  
   \textstyle\argmin_{D' \in \widetilde{\cX}^{*}}\widetilde{L}(D') \coloneqq
    % \argmin_{D'\in \cX^{*}} 
    \sum_{i\in [m]} \left(\hat{a}_i - \tilde{q}_i({D}') \right)^2
\end{align}



Since the new objective is differentiable everywhere in $\widetilde{\cX}^*$, we can run any first-order continuous optimization method to attempt to solve \eqref{eq:objectivediff}.
Were $\tilde{q}_i$  a good approximation for $q_i$ \emph{everywhere} in $\widetilde{\cX}$ for all queries $i\in[m]$, then the solution to \cref{eq:objectivediff} would approximate the solution to \cref{eq:objective}.
%
However, there are two other challenges that arise when we use the sigmoid approximation: flat gradients and near-threshold approximation quality. %First, flat gradients: 
If the sigmoid function has a large $\sigma$ (inverse temperature), its derivatives at points far from the threshold $\tau$ have small magnitudes. In other words, sigmoid approximations to linear threshold functions have nearly flat gradients far from the threshold. In the flat gradient regime, first order optimization algorithms fail because they get ``stuck''. This can be mitigated by using a small $\sigma$. But there is another issue: because threshold functions are discontinuous, any continuous approximation to a threshold function must be a poor approximation for points that are sufficiently close to the threshold. To make this poor approximation regime arbitrarily narrow, we would have to choose a large $\sigma$ 
% \gvdelete{sigmoid temperature}
, but this is in tension with the flat gradients problem mentioned earlier. As a result, it is not clear how to choose an optimal value for  $\sigma$ 
% \gvdelete{sigmoid temperature}
. %ahead of time, and indeed, we found that fixed choices of values of the sigmoid parameter had poor performance in practice because of one of these issues or the other. 

\input{docs/figures/sigmoid_plot/sigmmoid_neurips}
We overcome this issue by using a ``temperature annealing'' approach, described in detail in \cref{alg:oracle}.  Informally, we start with a small $\sigma$ 
% \gvdelete{sigmoid temperature}
, and run our optimization until the magnitude of the gradients of our objective function fall below a pre-defined threshold. At that point, we double $\sigma$
% \gvdelete{the sigmoid temperature}
and repeat, until convergence. The intuition behind this technique is that if the magnitude of the gradients has become small, we must be near a local optimum of the relaxed objective (\cref{eq:objectivediff}), since we have stopped making progress  towards the relaxed objective for the current value of $\sigma$. However, this might not be close to a local optimum of the actual objective function \cref{eq:objective}. By increasing $\sigma$ 
% \gvdelete{the sigmoid temperature}
at this stage, we make the relaxed objective a closer approximation to the real objective; we continue optimization until we are close to a local optimum of the new relaxed objective, and then repeat. We find that this annealing approach %has better optimization performance compared to any fixed setting of the Sigmoid parameter: see Figure \ref{fig:annealing}. 
worked well in practice. Figure \ref{fig:annealing} shows comparison of temperature annealing to optimization with fixed sigmoid temperature parameters. It can be seen that the annealing approach improves over every fixed setting of the parameter.


\input{docs/algos/oracle}
\input{docs/algos/raptor}

% We solve \cref{eq:objective} by continuous relaxation of the problem and applying gradient descent based optimization.
% Our algorithm handles marginal queries and threshold queries differently. For categorical data

% In this section we describe how to solve an optimization problem defined a follows. 
% Let $\cX$ be a mixed type data domain and let $D\in D^n$ be a dataset. 
% Given a set of threshold queries $Q$ and dataset $D$, let $\hat{a} \approx q(D)$ be an approximate answer vector of queries $Q$ about the dataset $D$.

%
% Then we want to efficiently generate a synthetic dataset $D'$ that solves following problem,
% %
% \begin{align} \label{eq:objective}
%   \min_{D'}\| \hat{a} - q(D') \|
% \end{align}
%  The objective \cref{eq:objective} is in general an intractable computation, since it is a minimization of a non-convex and non-differentiable objective.
 
%  and thus we use relax the problem by consider its differentiable using Sigmoid functions as surrogates for the threshold queries. For any $\sigma$ we define the following problem:
%  \begin{align}\label{eq:objectivediff}
%         \min_{D'} \| \hat{a}- \qtil(D', \sigma) \| 
%  \end{align}ws
 
%  In \cref{eq:objectivediff} we have a differentiable loss function that we can solve using Gradient descent (GD) based methods. Hence, the hope is that the optimal solution to Equation (2) gives a good solution to the objective in Equation (1).  However there are some challenges that we summarize as


% \begin{itemize}
%     \item Surrogate loss failure. 
%     \item  Flat/Diminishing Gradients.
% \end{itemize}



% In \cref{fig:barplots} we plot the error of a synthetic dataset generated by \cref{alg:oracle} to match the answers on a set of randomly generated threshold queries. The optimize queries sets with size $\{10, 100, 1000\}$, since in practice one rarely has to optimize over $1000$ queries. 
% We report the error of two different optimization algorithms. A naive optimization algorithm and and optimization algorithm that uses the different heuristics described in this section. 
% % We can see that \cref{alg:oracle} can accurately answers up to 10K randomly generated queries. 
% We use datasets Blobs and Adult.
% For the metrics we report both average and max error over the set of random queries. 


% \begin{figure}[b]
% \centering
% \centering
% \includegraphics[width=\textwidth]{images/opt_results.png}

% \caption{Optimization errors (max and mean) for both the Naive and the \textit{Dynamic-Sigmoid} algorithms, where each result is an aggregation over 10 runs . On each run optimizes over a fresh random sample of threshold queries, hence, the variance is over the randomness of the algorithm and the randomness of the query set sample. 
% The hyper-parameters are chosen as follows: The  number of epochs is set to 40 for both algorithms \sa{You are essentially running dynamic approach for longer epochs so I wonder if the difference would be reduced if you run the naive approach for more epochs?}. Further, both algorithms run a grid search over the learning rate parameter from the set $\{0.001, 0.01, 0.1 \}$ and choose the best result. The naive optimization tries all value of $\sigma_0$ in the set $\{5, 10, 15, 20, 25, 30,35, 40\}$ and reports the best result. The heuristics implementation always chooses $\sigma_0 = 0$ and $k=15$}.
% \label{fig:barplots}
% \end{figure}
